MLRegTest: A Benchmark for the Machine Learning of Regular Languages

Synthetic datasets constructed from formal languages allow fine-grained examination of the learning and generalization capabilities of machine learning systems for sequence classification. This article presents a new benchmark for machine learning systems on sequence classification called MLRegTest, which contains training, development, and test sets from 1,800 regular languages. Different kinds of formal languages represent different kinds of long-distance dependencies, and correctly identifying long-distance dependencies in sequences is a known challenge for ML systems to generalize successfully. MLRegTest organizes its languages according to their logical complexity (monadic second order, first order, propositional, or monomial expressions) and the kind of logical literals (string, tier-string, subsequence, or combinations thereof). The logical complexity and choice of literal provides a systematic way to understand different kinds of long-distance dependencies in regular languages, and therefore to understand the capacities of different ML systems to learn such long-distance dependencies. Finally, the performance of different neural networks (simple RNN, LSTM, GRU, transformer) on MLRegTest is examined. The main conclusion is that performance depends significantly on the kind of test set, the class of language, and the neural network architecture.

==> discussion-rand-adv.tex <==
\subsection{Comparing random and adversarial tests cases}

We determined ease of learning random strings vs. adversarial strings by aggregating together all models to compare the accuracy and f-scores across random and adversarial test sets, split into short and long strings. These results can be seen in figure \ref{tab:acc-and-f-scores}, showing that random data sets have much higher accuracy than the adversarial tests overall. This suggests that, while models overall were successful at finding items within a language, they nonetheless strugged to find the boundary between being in the language and being out of it. 

\begin{figure}
	\begin{tabular}{||l | r | r ||}
	   & \textsc{Accuracy} & \textsc{F-Scores} \\
	SR & .9180	       & .9178		   \\
	SA & .6758	       & .6767		   \\
	LR & .8773	       & .8727		   \\
	LA & .6600	       & .6547		   \\

	\end{tabular}
	\label{tab:RA-acc-and-f-scores}
	\caption{Mean accuracy and f-score or short and long random or adversarial test sets.}
\end{figure}

To verify the interpretation of these scores, we used a Wilcoxon test on all pairs of model accuracies, to ensure that they \footnote{not sure about phrasing here. Wilcoxon tests used to compare all means within each set and ensure a significant difference in set means?}. In all cases, models resulted in $p \langle 2.2e-16$. Finally, to determine a significant effect size, we determined Cohen's D for all pairs of models, as seen in figure \ref{tab:RA-cohens-d}. Cohen's $d$ measures the standard deviations in the overlap of each group. From these values, we can see that the effect size within model types (that is, both models are either random or adversarial) are below 0.3 standard deviations, which shows that the effect size of string length is small in this instance. On the other hand, when fixing string length and varying string type, models are above 1 standard deviation. 

\begin{figure}
	\begin{tabular}{|| c | c | c | c | c ||}
	   & SA	 & SR	       & LA 	     & LR 	   \\
	SA & \textendash & 1.467225    & 0.08365438  & 1.142367    \\
	SR & 1.467225    & \textendash & 1.6063      & 0.2793487   \\
	LA & 0.08365438  & 1.6063      & \textendash & 1.261733    \\
	LR & 1.142367    & 0.2793487   & 1.261733    & \textendash \\
	\end{tabular}
	\label{tab:RA-cohens-d}
	\caption{Absolute value of effect sizes for all pairs of models, as measured using Cohen's $d$. Pairs where the models are identical were not measured.}
\end{figure}
%I use the absolute values here, but in actuality, half of each pair of values is negative

Overall, this shows that the types of strings used in testing these models impact the accuracy of the results. Random string sets have a higher accuracy, while models have more difficulty in determining the border between languages. Effect size of the types of strings is much higher than the effect size of the string length. 
